Unsupervised Learning of Visual Features by Contrasting Cluster Assignments

Unsupervised image representations have significantly reduced the gap with supervised pretraining, notably with the recent achievements of contrastive learning methods. These contrastive methods typically work online and rely on a large number of explicit pairwise feature comparisons, which is computationally challenging. In this paper, we propose an online algorithm, SwAV, that takes advantage of contrastive methods without requiring to compute pairwise comparisons. Specifically, our method simultaneously clusters the data while enforcing consistency between cluster assignments produced for different augmentations (or views) of the same image, instead of comparing features directly as in contrastive learning. Simply put, we use a swapped prediction mechanism where we predict the cluster assignment of a view from the representation of another view. Our method can be trained with large and small batches and can scale to unlimited amounts of data. Compared to previous contrastive methods, our method is more memory efficient since it does not require a large memory bank or a special momentum network. In addition, we also propose a new data augmentation strategy, multi-crop, that uses a mix of views with different resolutions in place of two full-resolution views, without increasing the memory or compute requirements much. We validate our findings by achieving 75.3% top-1 accuracy on ImageNet with ResNet-50, as well as surpassing supervised pretraining on all the considered transfer tasks.

==> code.tex <==
\OURS is simple to implement and experiment with.
For this reason, we provide our \OURS implementation in PyTorch in this appendix.
%It is not a library, but simply a \texttt{main\_swav.py} importing model and criterion definitions with standard training loops.
From \texttt{main\_swav.py} are imported the dataset definition (\texttt{src/multicropdataset.py}), the model architecture (\texttt{src/resnet50.py}) and some miscellaneous training utilities (\texttt{src/utils.py}).
\\

For example, to train \OURS on a single node with 8 gpus for 400 epochs, run:
\\
\texttt{python -m torch.distributed.launch -{}-nproc\_per\_node=8 main\_swav.py \textbackslash \\}
\texttt{-{}-data\_path /path/to/imagenet \textbackslash \\}
\texttt{-{}-epochs 400 \textbackslash \\}
\texttt{-{}-base\_lr 0.6 \textbackslash \\}
\texttt{-{}-final\_lr 0.0006 \textbackslash \\}
\texttt{-{}-warmup\_epochs 0 \textbackslash \\}
\texttt{-{}-batch\_size 32 \textbackslash \\}
\texttt{-{}-size\_crops 224 96 \textbackslash \\}
\texttt{-{}-nmb\_crops 2 6 \textbackslash \\}
\texttt{-{}-min\_scale\_crops 0.14 0.05 \textbackslash \\}
\texttt{-{}-max\_scale\_crops 1. 0.14 \textbackslash \\}
\texttt{-{}-use\_fp16 true \textbackslash \\}
\texttt{-{}-freeze\_prototypes\_niters 5005 \textbackslash \\}
\texttt{-{}-queue\_length 3840 \textbackslash \\}
\texttt{-{}-epoch\_queue\_starts 15 \textbackslash \\}

Our best ResNet-50 \OURS model is available to download at \url{https://dl.fbaipublicfiles.com/deepcluster/swav_800ep_pretrain.pth.tar}.

\pythonexternal{main_swav.py}

\pythonexternal{src/multicropdataset.py}

\pythonexternal{src/resnet50.py}

\pythonexternal{src/utils.py}

